DarSwin: Distortion Aware Radial Swin Transformer

Wide-angle lenses are commonly used in perception tasks requiring a large field of view. Unfortunately, these lenses produce significant distortions, making conventional models that ignore the distortion effects unable to adapt to wide-angle images. In this paper, we present a novel transformer-based model that automatically adapts to the distortion produced by wide-angle lenses. Our proposed image encoder architecture, dubbed DarSwin, leverages the physical characteristics of such lenses analytically defined by the radial distortion profile. In contrast to conventional transformer-based architectures, DarSwin comprises a radial patch partitioning, a distortion-based sampling technique for creating token embeddings, and an angular position encoding for radial patch merging. Compared to other baselines, DarSwin achieves the best results on different datasets with significant gains when trained on bounded levels of distortions (very low, low, medium, and high) and tested on all, including out-of-distribution distortions. While the base DarSwin architecture requires knowledge of the radial distortion profile, we show it can be combined with a self-calibration network that estimates such a profile from the input image itself, resulting in a completely uncalibrated pipeline. Finally, we also present DarSwin-Unet, which extends DarSwin, to an encoder-decoder architecture suitable for pixel-level tasks. We demonstrate its performance on depth estimation and show through extensive experiments that DarSwin-Unet can perform zero-shot adaptation to unseen distortions of different wide-angle lenses. The code and models are publicly available at https://lvsn.github.io/darswin/

==> Sections_workshop/abstract_workshop.tex <==
\begin{abstract}
Wide-angle lenses are commonly used in perception tasks requiring a large field of view. Unfortunately, these lenses produce significant distortions making conventional models that ignore the distortion effects unable to adapt to wide-angle images. In this paper, we present a novel transformer-based model that automatically adapts to the distortion produced by wide-angle lenses. We leverage the physical characteristics of such lenses, which are analytically defined by the radial distortion profile (assumed to be known), to develop a distortion aware radial swin transformer (DarSwin). 
We validate our method on classification tasks using synthetically distorted ImageNet data and show through extensive experiments that DarSwin can perform zero-shot adaptation to unseen distortions of different wide-angle lenses. Compared to other baselines, DarSwin achieves the best results (in terms of accuracy) with significant gains when trained on bounded distortions levels (very-low, low, medium, and high) and tested on all including out-of-distribution distortions. 
%
%(1-4\% and 20\%) respectfully to the best baseline.
%We validate our method on classification tasks using synthetically distorted ImageNet data and show through extensive experiments that DarSwin can perform zero-shot adaptation to unseen distortions of different wide-angle lenses. Compared to other baselines, DarSwin achieves the best results (in terms of Top-1), when tested on out of distribution distortion with almost 20\% gain in top-1 accuracy in "very low" distortion and (1-4 \%) gain in "low", "medium" and "high" distortions from the second best baseline. 
\end{abstract}

==> Sections_workshop/background_workshop.tex <==
\section{Image formation}
\label{sec:background}

\begin{figure*}[!ht]
\centering
\includegraphics[width=\linewidth]{Figures/Darswin/Darswin_arch.pdf}
\caption[]{Overview of our distortion aware transformer architecture, \thename (Azimuth Merge). It employs hierarchical layers of Swin-S transformer blocks~\cite{liu2021swin} interspersed with patch merging layers. To make it adapt to lens distortion, the patch partition, linear embedding, and patch merging layers all take the lens projection curve $\mathcal{P}$ (c.f. \cref{sec:background}) as input.}
\label{fig:darswin-arch}
\end{figure*}

We begin with a brief review of lens distortion models relevant to this work. The pixel coordinates $\mathbf{p}_\mathrm{im}$ of a 3D point $\mathbf{p}_\mathrm{w} = [x, y, z]^\mathsf{T}$ in world coordinates are given by $\mathbf{p}_{\mathrm{im}} = [u, \; v]^\mathsf{T} = \mathcal{P}(\mathbf{p}_{\mathrm{w}}) \,,$
%
% \begin{equation}
% \mathbf{p}_{\mathrm{im}} = [u, \; v]^\mathsf{T} = \mathcal{P}(\mathbf{p}_{\mathrm{w}}) \,,
% \label{eq:formation-cartesian}
% \end{equation}
%
where $\mathcal{P}$ is a 3D-to-2D projection operator, including conversion from homogeneous coordinates to 2D. Here, without loss of generality, the camera is assumed to be at the world origin (so its rotation and translation are ignored).
% To represent wide-angle images, it is common practice to use a projection model that describes the relationship between the radial distance $r_\mathrm{im} = \sqrt{u^2 + v^2}$ from the image center and the incident angle $\theta = \arctan ( \nicefrac{\sqrt{x^2 + y^2}}{z} )$. This relationship takes the generic form
% %
% \begin{equation}
% r_{\mathrm{im}} = \mathcal{P}(\theta) \,.
% \label{eq:formation-radial}
% \end{equation}
% %
Within the scope of our interest, we consider two types of projections.

\begin{itemize}
\item Under the \textbf{perspective projection model}, the projection operator $\mathcal{P}$ takes the form $\mathcal{P}_\mathrm{pers}(\theta) \equiv r_{\mathrm{im}} = f \tan (\theta) \,,$
%
% \begin{equation}
% \mathcal{P}_\mathrm{pers}(\theta) \equiv r_{\mathrm{im}} = f \tan (\theta) \,,
% \end{equation}
%
where $f$ is the focal length, $r_{im} = \sqrt{u^2 + v^2}$ is the radial distance and $\theta = \arctan ( \nicefrac{\sqrt{x^2 + y^2}}{z} )$ is the incident angle. The perspective projection is the rectilinear model of pinhole lenses. Wide-angle lenses disobey this law and therefore cause non-linear distortions.   
\item The \textbf{spherical projection model}~\cite{barreto2006unifying,mei2007single} describes the radial distortion by a \emph{single}, \emph{bounded} parameter $\xi \in [0, 1]$\footnote{$\xi$ can be slightly greater than 1 for certain types of catadioptric cameras~\cite{ying2004consider} but this is ignored here.}. It projects the world point $\mathbf{p}_{\mathrm{w}}$ to the image as $[u, v]^\mathsf{T} = \left[ \frac{xf}{\xi ||\mathbf{p}_\mathrm{w}||+z},\frac{yf}{\xi ||\mathbf{p}_\mathrm{w}||+z} \right]^\mathsf{T} .$ We employ this model in experiments (\cref{sec:experiments}) because of its ability to represent distortion with a single parameter.
\end{itemize}
%%%%%%%%%%%%%%%%%%%%
% \paragraph{Perspective projection.}
% Under the perspective projection model, the projection operator $\mathcal{P}$ takes the form \cite{kannala2006generic} $\mathcal{P}_\mathrm{pers}(\theta) \equiv r_{\mathrm{im}} = f \tan (\theta) \,,$
% %
% % \begin{equation}
% % \mathcal{P}_\mathrm{pers}(\theta) \equiv r_{\mathrm{im}} = f \tan (\theta) \,,
% % \end{equation}
% %
% where $f$ is the focal length (in pixels), $r_{im} = \sqrt{u^2 + v^2}$ is the radial distance and $\theta = \arctan ( \nicefrac{\sqrt{x^2 + y^2}}{z} )$ is the incident angle. The perspective projection is the rectilinear model of pinhole lenses. Wide-angle lenses disobey the law of perspective projection and therefore cause non-linear distortions.   

% \paragraph{Polynomial projection.}
% In the case of wide-angle lenses, there are several classical projection models \cite{beck1925apparatus,hill1924lens,fleck1995perspective,miyamoto1964fisheye} giving different formulas for $\mathcal{P}$; see \cite{hughes2010accuracy} for a detailed analysis of the accuracy of such models. A unified, more general, model is defined as an $n-$degree polynomial and given by
% %
% \begin{equation}
% \mathcal{P}_\mathrm{poly}(\theta) \equiv r_{\mathrm{im}} = a_1\theta + a_2\theta^2 + ... + a_n \theta^n \,.
% \end{equation}
% %
% For example, the WoodScape dataset~\cite{yogamani2019woodscapes} employs a 4-degree ($n=4$) polynomial for their lens calibration. We adopt this polynomial function to define the lens projection curve used in our method (\cref{sec:methodology}).
%%%%%%%%%%%%%%%%%%%%%
% \paragraph{Spherical projection.} The spherical projection model~\cite{barreto2006unifying,mei2007single} describes the radial distortion by a \emph{single}, \emph{bounded} parameter $\xi \in [0, 1]$\footnote{$\xi$ can be slightly greater than 1 for certain types of catadioptric cameras~\cite{ying2004consider} but this is ignored here.}. It projects the world point $\mathbf{p}_{\mathrm{w}}$ to the image as $[u, v]^\mathsf{T} = \left[ \frac{xf}{\xi ||\mathbf{p}_\mathrm{w}||+z},\frac{yf}{\xi ||\mathbf{p}_\mathrm{w}||+z} \right]^\mathsf{T} .$
%
%\begin{equation}
%%\resizebox{0.91\hsize}{!}{%
%% \resizebox{0.91\hsize}{!}{
%\mathcal{P}_\mathrm{s}(\mathbf{p}_\mathrm{w}) \equiv [u, v]^\mathsf{T} = \left[ \frac{xf}%%{\xi ||\mathbf{p}_\mathrm{w}||+z},\frac{yf}{\xi ||\mathbf{p}_\mathrm{w}||+z} %\right]^\mathsf{T} \,.
%% .
%\label{eqn:sphproj}
%\end{equation}
%%%%%%%%%%%%%%%%%%%
% \begin{equation}
% %\resizebox{0.91\hsize}{!}{%
% % \resizebox{0.91\hsize}{!}{
% [u, v]^\mathsf{T} = \left[ \frac{xf}{\xi ||\mathbf{p}_\mathrm{w}||+z},\frac{yf}{\xi ||\mathbf{p}_\mathrm{w}||+z} \right]^\mathsf{T} \,.
% % .
% \label{eqn:sphproj}
% \end{equation}
%%%%%%%%%%%%%%%%%%%

%
% As mentioned, one of the advantages of the spherical model is the closed-form solution of the inverse projection equation. This inverse projection is especially useful when applying the spherical lens model to panoramic images (see sec.~\ref{sec:dataset_generation}). Given a 2D image point $\mathbf{p}_\mathrm{im}=[u, v]^\mathsf{T}$, the back-projection from the image to the sphere is computed by $\mathbf{p}_\mathrm{s} = [\omega u, \; \omega v, \; \omega \! - \! \xi]^\mathsf{T}$, where
% %
% \begin{equation}
% \omega = \frac{\xi + \sqrt{1 + (1-\xi^2)(u^2+v^2)}}{u^2+v^2+1} \,.
%   \label{Eq::backPro}
% \end{equation}
% %
% We can also derive the equation for the effective horizontal field of view $h_\theta$, noting $\hat{u} = -u_0/f$: 
% %
% \begin{equation}
% h_{\theta} = 2\arccos{\left(\frac{\xi+\sqrt{1+(1-\xi^2)\hat{u}^2}}{\hat{u}^2+1} - \xi\right)} \,.
% \end{equation}
% %
% Please refer to the supplementary material for more details. 

% \subsection{Swin transformer}

\begin{figure}[h!]
  \centering
  \includegraphics[width=0.65\linewidth]{Figures/Darswin/Patch_partition.pdf}
  \caption{Example of distortion aware polar patch partition. Here, $N_r=4$ and $N_\varphi = 4$ partitions along radius and azimuth respectively are used to illustrate (right, only the top-right quadrant of the image is shown). While the azimuth partitioning is performed in an equiangular fashion, the radial dimension takes the lens distortion curve (left) into account. The field of view along the incident angle $\theta$ is split into $N_r$ equal parts (left) and corresponding radial are obtained from the distortion curve. Hence for different lenses we can have different radii depending on the distortion parameters. }
  \label{fig:patch-partition}
\end{figure}


==> Sections_workshop/classification_workshop.tex <==
\section{Classification experiments}
\label{sec:experiments}

We perform a series of experiments on image classification to evaluate the efficacy of our proposed method. Due to the lack of classification dataset for wide-angle images, we instead create synthetically distorted images using 200 randomly chosen classes from the ImageNet1k dataset~\cite{krizhevsky2012classif}. To evaluate our approach on a wide range of conditions, we employ the unified spherical projection model (c.f. \cref{sec:background}) to synthetically distort the (perspective) ImageNet1k images.

% We conduct experiments on a subset of synthetically distorted ImageNet1k dataset \cite{imagenet} using spherical projection model c.f. \cref{sec:background} with 200 classes. 


\subsection{Dataset}
\label{sec:dataset}
%
\paragraph{Training sets/Test sets} We generate four different training sets withdifferent levels of distortion, defined by the distortion parameter $\xi$: ``very low'' ($\xi \in [0.0, 0.05]$), ``low'' ($\xi \in [0.2, 0.35]$), ``medium'' ($\xi \in [0.5, 0.7]$), and ``high'' ($\xi \in [0.85, 1.0]$). \Ak{(for more information refer fig. 2 in supplementary)}. Training images are distorted on-the-fly during training with the distortion level sampled uniformly from the interval mentioned above. Each training set contains 260,000 images and 10,000 validation images, over 200 classes. \textbf{Test set} consists of 30,000 images over 200 classes.
%


%are generated using the same procedure. Here, $\xi$ is determined once for each image and kept fixed. And we test for all $\xi$ values between $[0, 1]$ to evaluate generalization to different lens distortions.%\todo{This last sentence does not agree with what we say in \cref{sec:generalization-results}.}


% \Ak{ We generate four different test sets for four different levels of distortion from ”very low” to ”high”. Each set contains 30,000 images over 200 classes, in which a different distortion parameter $\xi$ is fixed for all samples in that test set.}

% We generate four different test sets 
%  for four different levels of distortion from "very low" to "high". Each set has 30,000 images across the 200 classes. }

% \paragraph{Test set} We generate four different test sets 
% for four different levels of distortion from "very low" to "high". Each set has 30,000 images across the 200 classes. Unlike in training distortion where we sample distortion on-the-fly, for each image in the test set the distortion parameter $\xi$ is fixed. 

%%%%%%%%%%%%%%%%%%%%%%%%%% change %%%%%%%%%%%%%%%%%%%%%%%%%% 
% \begin{figure}
% \footnotesize
% \setlength{\tabcolsep}{1pt}
% \begin{tabular}{cccc}
% Very low & Low & Medium & High \\
% \includegraphics[width = 0.24\linewidth]{Figures/Classification/little_distorted.png} &
% \includegraphics[width = 0.24\linewidth]{Figures/Classification/low_distorted.png} &
% \includegraphics[width = 0.24\linewidth]{Figures/Classification/medium_distorted.png} &
% \includegraphics[width = 0.24\linewidth]{Figures/Classification/high_distorted.png} \\
% \includegraphics[width = 0.24\linewidth]{Figures/Classification/little_undistorted.png} &
% \includegraphics[width = 0.24\linewidth]{Figures/Classification/low_undistorted.png} &
% \includegraphics[width = 0.24\linewidth]{Figures/Classification/medium_undistorted.png} &
% \includegraphics[width = 0.24\linewidth]{Figures/Classification/high_undistorted.png}
% \end{tabular}
% \caption{Visualization of a checkerboard pattern distorted according to each distortion level at its original resolution of (224, 224) and downsampled to (64, 64) in our four training sets. From left to right: very low, low, medium, and high. The second row represents the respective undistorted images.}
% \label{fig:distortion-levels}
% \end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%% change %%%%%%%%%%%%%%%%%%%%%%%%%% 

\subsection{Baselines}
\label{sec:baselines}

We compare our approach with the following baselines: Swin-S~\cite{liu2021swin}, Deformable Attention Transformer (DAT-S)~\cite{xia2022vision}, and Swin-S on input undistorted images dubbed ``Swin(undis)''. As with our DarSwin, this last baseline has knowledge of the distortion parameters whereas the first two do not. Note that we do not include comparisons to methods which estimate distortion \cite{yin2018fisheyerectnet, xue2019learning, 9980359, zhang2015line}. Indeed, the spherical projection model (\cref{sec:background}) is bijective: the undistortion function has a closed form and is exact. Therefore, the ``Swin (undis)'' method serves as an upper bound to all self-calibration methods because it is, in essence, being given the ``ground truth'' undistortion.
%\Ak{Training details in supplimentary}


% All three baselines employ 32 divisions along the image width and height. For DarSwin, we use $N_r = 16$ and $N_\varphi = 64$ divisions along the radius and azimuth respectively, which yields the same total number of 1024 patches for all methods. All three baselines are trained with a window size (4, 4) on our synthetically distorted training sets.

% All methods use the AdamW optimizer on a batch size of 128 using a cosine decay learning rate scheduler and 20 epochs of linear warm-up. We use an initial learning rate of 0.001 and a weight decay of 0.05. We include all of the augmentation and regularization strategies of \cite{liu2021swin}, except for random crop and geometric transformation (like shearing and translation). Our model requires 0.03M additional parameters over the Swin baseline which contains 48M, representing a 0.061\% increase.
% \Ak{But, our model is more complex by ; both models have approximately 48M parameters, but our model has $\sim$0.03M (29862) extra parameters due to the linear embedding sampling layer.}

% \subsection{Results}

% \paragraph{Classification accuracy} We begin by reporting the top-1 and top-5 classification accuracies of baselines and our model trained and tested on same distortion level in \cref{tab:distortion_results_table}. We note that Swin (undis) and DAT outperform our model when trained on very low distortion levels, as the images in these regions are nearly perspective (c.f. \cref{fig:distortion-levels}). As models are trained on higher distortion levels, our model outperform the baselines in almost all scenarios.



% \begin{table*}
% \centering
% \footnotesize
% \caption{Comparisons of top-1 and top-5 accuracies of the models trained on distortion levels of distortion (pink region in \cref{fig:results-distortion}) and tested on distortion level $\xi = 0.4$. Each row is color-coded as \colorbox{best}{best} and \colorbox{second}{second best}.}
% % \resizebox{\columnwidth}{!}{%
% % \setlength{\tabcolsep}{0.02em}
% \begin{tabular}{lcccccccc}
% \toprule
%             & \multicolumn{2}{c}{Very Low} & \multicolumn{2}{c}{Low} & \multicolumn{2}{c}{Medium} & \multicolumn{2}{c}{High}\\
% Method      & Top-1    & Top-5   & Top-1   & Top-5   & Top-1  & Top-5   & Top-1   & Top-5   \\
% \midrule
% DarSwin     & \cellcolor{best}{75.6}\%   & \cellcolor{best}{92.0}\%  & \cellcolor{best}{91.4}\%  & \cellcolor{second}{97.2}\%  & \cellcolor{best}{91.0}\% & \cellcolor{best}{97.0}\%  & \cellcolor{best}{88.4}\%  & \cellcolor{best}{96.4}\% \\
% Swin        & 33.9\%   & 59.1\%  & 85.0\%  & 95.1\%  & 78.7\% & 92.8\%  & 40.1\%  & 65.5\% \\
% Swin (undis) & \Ak{46.9}\%   & \Ak{70.7}\%  & \Ak{90.1}\%  & \cellcolor{best}{\Ak{97.3}}\%  & \cellcolor{second}{\Ak{88.9}}\% & \cellcolor{second}{\Ak{96.5}}\%  & \cellcolor{second}{\Ak{80.3}}\%  & \cellcolor{second}{\Ak{93.8}}\% \\
% DAT         & \cellcolor{second}{57.5}\%   & \cellcolor{second}{80.2}\%  & \cellcolor{second}{90.4}\%  & 96.6\%  & 88.5\% & 95.8\%  & 75.7\%  & 91.9\% \\
% \bottomrule
% \end{tabular}
% % }
% \label{tab:distortion_results_table}
% \end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[!h]
\centering
\footnotesize
\caption{Comparisons of top-1 accuracy of the models trained on four levels of distortion (pink regions in \cref{fig:results-distortion}) and tested on distortion level $\xi = 0.4$. Each row is color-coded as \colorbox{best}{best} and \colorbox{second}{second best}.}
\begin{tabular}{@{}ccccc@{}}
\toprule
Methods      & Very Low & Low  & Medium & High \\ \midrule
DarSwin      & \cellcolor{best}{80.33}   & \cellcolor{best}{92.61}  & \cellcolor{best}{92.35}   & \cellcolor{best}{91.39} \\
Swin     & 33.94     & 87.90 & 78.7   & 40.1 \\
Swin (undis) & 47.48     & \cellcolor{second}{91.52} & \cellcolor{second}{91.07}   & \cellcolor{second}{87.34} \\
DAT          &  \cellcolor{second}{57.5}  & 90.4 & 88.5   & 75.7 \\ \bottomrule
\end{tabular}
\label{tab:distortion_results_table}
\end{table}

\subsection{Zero-shot lens distortion generalization} 
\label{sec:generalization-results}

We are interested in evaluating whether our distortion-aware method can better generalize to other unseen lenses at test time. Hence, we train each approach on a level of distortion (c.f. \cref{sec:dataset}) and evaluate them on all distortion values $\xi \in [0, 1]$. For this, entire test set is distorted using a single $\xi$ value, and we repeat this process for every $\xi \in [0, 1]$ to simulate different lens distortion. %\todo{exactly how? Previous text was very unclear.}. 

Results are reported in \cref{fig:results-distortion}, where the distribution of training distortions is drawn in pink. We observe that \thename shows much greater generalization capabilities outside of the training domain. Furthermore, \cref{tab:distortion_results_table} shows the top-1 accuracy for the test set distorted with $\xi = 0.4$, which is in none of the training intervals. Again, we note that \thename yields better generalization accuracy (without fine-tuning) than all baselines, even Swin (undis) which also has access to the ground truth distortion function (see \cref{sec:baselines}). 

% While overall classification accuracy is important, we are mostly interested in evaluating whether our distortion aware method can better generalize to other lenses at test time. Here, we perform zero-shot generalization by training on a single level of distortion, and testing (without any additional finetuning) on other distortion levels. \Cref{fig:results-distortion} shows the generalization of our method across all values of $\xi \in [0,1]$ using top-1 accuracy. The pink region indicates the training distortion levels described in \cref{tab:distortion_results_table}. 



% Even though the baseline methods perform better initially on ``very low'' and ``low'' distortion levels (\cref{fig:results-distortion}a-b), our model adapts far better as the test distortion changes. In the ``medium'' and ``high'' distortion training models (\cref{fig:results-distortion}c-d), our model outperforms Swin and DAT, but in the low region of distortion, our method is comparable to Swin (undis). We think that our method generalizes better than the baselines due to the presence of lens information embedded into DarSwin.





==> Sections_workshop/discussion_workshop.tex <==
%!TEX root = ../main.tex
\section{Discussion}
\label{sec:Discussion}

This paper presents \thename, a new distortion aware vision transformer which adapts its structure to the lens distortion profile of a (calibrated) lens. \thename achieves state-of-the-art performance on zero-shot adaptation (without pretraining) on different lenses on classification using synthetically distorted images from the ImageNet1k dataset. 
% \paragraph{Limitations and future research directions} While our method demostrates state-of-the-art performance, it suffers from some limitations. First, the distortion aware sampling strategy is shown to be effective for zero-shot adaptation, the sparsity of sampling points and necessity to interpolate pixel values may affect the performance of the model. While this issue is partially alleviated using our proposed jittering augmentation technique, other strategies may also be possible. Second, our model assumes knowledge of the lens distortion profile, hence it is appropriate only for the calibrated case. We hope to extend our work to uncalibrated lenses, for example by taking inspiration from \cite{Hold-Geoffroy_2018_CVPR, yin2018fisheyerectnet, article1}. Finally, while our experiments demonstrate promising performance on classification experiments, we wish to expand to per-pixel tasks, such as semantic classification and depth estimation. Here, making pixel decoders distortion aware is an exciting direction for future work. 

% We hope that the strong performance of \thename's  as an encoder will inspire insights towards designing distortion aware models for un-calibrated lenses and for dense pixel-level classification tasks.


==> Sections_workshop/introduction_workshop.tex <==
\section{Introduction}


% \begin{figure}[t] 
%     \centering
%     \footnotesize
%     \setlength{\tabcolsep}{1pt}
%     \begin{tabular}{cccc} 
%     % \quad \quad \rotatebox{90}{\footnotesize{attention maps} \quad \ \  \ \ \ \ \  \ \ \  \ \ \ \ \ \  \footnotesize{tokenization}   \quad   \ \ \ \ \ \ \ \ \ \ \ \ \  \ \ \footnotesize{input} }   
%     \includegraphics[width=0.99\linewidth, angle=0]{Figures/TeaserFigIntro.pdf} \\
%     \ \ \   \rotatebox{0}{\footnotesize{Swin~\cite{liu2021swin}} \quad \ \  \ \ \ \  \quad  \quad  \quad  \quad    \quad  \quad  \quad   \quad  \quad  \quad  \quad \quad \      \footnotesize{DarSwin} (ours)  }   \\     
%     \end{tabular}
%     \caption[]{Illustration of (cartesian) Swin~\cite{liu2021swin} (left) and our (radial) \thename (right) given a wide-angle image (middle). While Swin~\cite{liu2021swin} computes the predefined shifted windows over square image patches, \thename performs radial transforms using distortion aware patch partitions modules which enables greater generalization capabilities across different lenses.}
%     \label{fig:teaser}
% \end{figure}

Wide field of view (FOV) lenses are becoming increasingly popular because their increased FOV minimizes cost, energy, and computation since fewer cameras are needed to image the entire environment.
They are having a positive impact on many applications, including security ~\cite{kim2015fisheye}, augmented reality (AR)~\cite{schmalstieg2017ar}, healthcare and more particularly, autonomous vehicles \cite{deng2019restricted,yogamani2019woodscapes}, which require sensing their surrounding $360^{\circ}$ environment.
\begin{figure}[t] 
    \centering
    \footnotesize
    \setlength{\tabcolsep}{1pt}
    \begin{tabular}{cccc} 
    % \quad \quad \rotatebox{90}{\footnotesize{attention maps} \quad \ \  \ \ \ \ \  \ \ \  \ \ \ \ \ \  \footnotesize{tokenization}   \quad   \ \ \ \ \ \ \ \ \ \ \ \ \  \ \ \footnotesize{input} }   
    \includegraphics[width=0.99\linewidth, angle=0]{Figures/Teaser_fig_ak.pdf} \\
    \ \ \   \rotatebox{0}{\footnotesize{ \quad Swin~\cite{liu2021swin}} \quad \ \  \ \ \ \  \quad  \quad  \quad  \quad    \quad  \quad  \quad   \quad  \quad   \quad \quad \      \footnotesize{DarSwin} (ours)  }   \\     
    \end{tabular}
    \caption[]{Illustration of (cartesian) Swin~\cite{liu2021swin} (left) and our (radial) \thename (right) given a wide-angle image (middle). While Swin~\cite{liu2021swin} computes attention on the predefined windows over square image patches (bottom left orange region), \thename performs radial transformations using distortion-aware radial patches and computes the attention on windows defined over radial patches (shown in orange region bottom right), which enables greater generalization capabilities across different lenses.}
    \label{fig:teaser}
\end{figure}

Unfortunately, such wide angle lenses create significant distortions in the image since the perspective projection model no longer applies: straight lines appear curved, and the appearance of the same object changes as a function of its position on the image plane. This distortion breaks the translation equivariance assumption implicit in convolution neural networks (CNNs) and therefore limits their applicability. This problem is further exacerbated by the diversity in lens distortion profiles: as we will demonstrate, a network naively trained for a specific lens tends to overfit to that specific distortion, and does not generalize well when tested on another lens. Just as methods are needed to address the ``domain gap''~\cite{huang2018multimodal} from dataset bias~\cite{torralba2011unbiased,khosla2012undoing}, we believe we must also bridge the ``distortion gap'' to truly make wide angle imaging applicable.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% One popular strategy to bridge the distortion gap is to cancel the effect of distortion on the image plane by warping the input image back to a perspective projection model according to calibrated lens parameters. Conventional approaches can then be trained and tested on the resulting ``un-distorted'' images. Unfortunately, warping a very wide angle image to a perspective projection tends to create severely stretched images and restricts the maximum field of view since, in the limit, a point at \ang{90} azimuth projects at infinity.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{figure}[t] 
%     \centering
%     \footnotesize
%     \setlength{\tabcolsep}{1pt}
%     \begin{tabular}{cccc} 
%     \quad \quad \rotatebox{90}{\footnotesize{attention maps} \quad \ \  \ \ \ \ \  \ \ \  \ \ \ \ \ \  \footnotesize{tokenization}   \quad   \ \ \ \ \ \ \ \ \ \ \ \ \  \ \ \footnotesize{input} }   
%     \includegraphics[width=0.90\linewidth, angle=0]{Figures/DarSwinTeaserFig.pdf} \\
%     \ \  \ \ \ \ \  \ \ \ \ \  \rotatebox{0}{\footnotesize{Swin~\cite{liu2021swin}} \quad \ \  \ \ \ \  \quad \      \footnotesize{DarSwin} (ours)    \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \  \ \ \footnotesize{ViT~\cite{dosovitskiy2020vit} } }  \\
%     % &   \includegraphics[width=0.51\linewidth, angle=0]{figures_and_plots/figures/ours_minsum.pdf}\\ 
%     % \includegraphics[width=0.47\linewidth, angle=0]{figures_and_plots/figures/ours_minsum.pdf}\\  
%     % (a) Three baseline methods   & \quad   (b) Set matching with sum-min \\       
%     \end{tabular}
%     \caption[]{Illustration of our radial DarSwin (middle) versus Cartesian methods Swin~\cite{liu2021swin} (right) and ViT~\cite{dosovitskiy2020vit} (left)   given a wide-angle image of turtle at the top row.  While Swin~\cite{liu2021swin} computes the predefined shifted windows over the image patches to increase the efficiency in self-attention computations, ViT~\cite{dosovitskiy2020vit} naively computes the self-attention over all of the patches. In contrast to the Cartesian methods, DarSwin, with its distortion aware patch partitions and jittering sampling modules, enables us to perform radial transforms for appropriate adaptations in a single-shot scenario without pre-training. From a patch and window size perspective, nevertheless, a careless design of the Swin~\cite{liu2021swin} would result in undersampling (high data would require to better performance) while ViT~\cite{dosovitskiy2020vit} would potentially result in oversampling (high computation cost). Taking the benefits from the best of two worlds, our radial DarSwin similar to ViT~\cite{dosovitskiy2020vit} could extend to every part of the input image during the adaptation, but in a more effective manner akin to Swin~\cite{liu2021swin}.   
%     }
%     \label{fig:DarSwin_teaser}
% \end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Vision transformers~\cite{dosovitskiy2020vit} and their more recent variants~\cite{zhou2021deepvit,liu2021swin,xia2022vision} could also better bridge the ``distortion gap'' since they do not assume any prior structure other than permutation equivariance, but their cartesian partitioning of the image plane do not take lens geometry into account (see \cref{fig:teaser}).

% % \ola{Motivate transformers first - introduce the meth{}od second} 
% In this paper, we present \thename, a transformer-based architecture that adapts its structure to the lens distortion profile, which is assumed to be known (i.e. the camera is calibrated). Our method, inspired by the recent Swin transformer architecture~\cite{liu2021swin}, leverages a distortion aware sampling scheme for creating token embeddings, employs polar patch partitioning and merging strategies, and relies on angular relative positional encoding. %We have also investigated an alternative position encoding strategy based on polar coordinates~\cite{ning2020polar}. 
% This explicitly embeds knowledge of the lens distortion in the architecture and makes it much more robust to the ``distortion gap'' created by training and testing on different lenses. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% In this paper, we present \thename: a transformer-based architecture that adapts its structure to the lens distortion profile, which is assumed to be known (calibrated). \thename aims at radial representation learning to generalize on wide-angle images that have radial structures rather than the generic Cartesian inputs. Therefore, the application of our method can extend from classification to segmentation of radial inputs such as wide-angle images. Inspired by the recent Swin transformer architecture~\cite{liu2021swin}, our \thename is a ``distortion aware'' method that enables radial patch partitioning and merging strategies. 

The main contribution of this paper is a novel transformer-based encoder that automatically adapts to the (known) lens distortion profile, which relies on a combination of the following novel distortion aware components: polar patch partitioning, distortion-based sampling scheme for creating token embeddings along with a jittering technique for better generalization, and angular relative position encoding for radial patch merging.
We show, through extensive classification experiments, that \thename can perform zero-shot adaptation (without pretraining) across different lenses. Indeed, when our method is trained on a restricted set of distortions, we observe that it is much more robust to changes in distortions at test time than all of the compared alternatives, including baseline Swin~\cite{liu2021swin} (applied on both distorted and undistorted images) and deformable attention transformer ~\cite{xia2022vision}. 

% We also demonstrate similar generalization behavior on semantic segmentation on wide-angle images.   \todo{Can we better quantify performance here}.\ola{To add the accuracy gain (in \%) for classification and pixel accuracy (IoU) for segmentation}


% \begin{figure}[t]
%   \centering
%   %\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%   % \includegraphics[width=1.0\linewidth]{images/teaser.pdf}
%   \todo{Add teaser.}
%   \caption{\todo{Write teaser caption.}}
%   \label{fig:teaser}
% \end{figure}



% To overcome this, some rectification networks \cite{calistraight, calirect} use neural networks to predict the distortion parameter of the lens and use them to cancel the effect of distortion. but they lose some information in the process. 


% We propose a method based on transformer networks that can adapt to multiple distortion profiles. A naive reason to choose transformer as our base network is due to the fact that transformers have more degrees of freedom in transformer compared to other architecture, i.e. transformer doesn't assume any prior structure other than permutation equivariance, any other structure has to be provided using positional encoding.

% We build our model on the current state-of-the-art Swin transformer~\cite{liu2021swin}. But, all the vision transformer-based architecture like \cite{dosovitskiy2020vit,zhou2021deepvit,touvron2021deit,lin2017fpn} including Swin~\cite{liu2021swin}, uses grid structure to define patches of images for token embeddings, to get a CNN-like structure and have translation equivariance, but as we discussed earlier translation equivariance is not enough for fisheye images. So we tried to warp this grid structure to define radial patches as shown in \cref{fig:swinvdarswin2}, we define these radial patches by using polar coordinates instead of Cartesian. we believe by using radial patches we can introduce a rotational symmetry along with translation by moving along azimuth and radius simultaneously, In addition to that, we use the fisheye lens curve as shown in \cref{fig:teaser} to our advantage by guiding the divisions along the radius, making it distortion aware in the process.


% Ma et al.~\cite{ma_defocus_2022} did this and that. \Cref{fig:teaser} shows blah.  In \cref{fig:teaser}, blah. 

% \begin{figure}
% Beautiful teaser. 
% \caption{Beautiful teaser, I told you!}
% \label{fig:teaser}
% \end{figure}

==> Sections_workshop/method_workshop.tex <==
\section{Methodology}
\label{sec:methodology}



\subsection{Overview}

\Cref{fig:darswin-arch} shows an overview of our proposed distortion aware transformer architecture. It accepts as input a single image and its distortion parameters in the form of a lens projection curve $\mathcal{P}(\theta)$. The image domain is first segmented into patches according to a polar partitioning module (\cref{sec:polar-partition}). Then, a linear embedding is computed from sampled points (\cref{sec:linear-embedding}), reshaped into a radial-azimuth projection and fed to the first Swin transformer block. The attention mechanism employs an angular relative positional encoding scheme guided by the lens curve. This is followed by three blocks performing patch merging (\cref{sec:patch-merging}) and additional Swin transformer blocks. More details are provided below.


\subsection{Polar partition}
\label{sec:polar-partition}

The first step of our proposed architecture is to partition the image (defined by a 2D plane) into patches. As opposed to Swin which performs the split in cartesian coordinates, \thename employs a polar patch partitioning strategy as shown in \cref{fig:teaser}. After centering a polar coordinate system on the image center (assumed to be known), we first split according to azimuth angle $\varphi$ (in the image plane) in $N_\varphi$ equiangular regions. For the radial dimension, we split the image into $N_r$ radial regions such that the splits are equiangular in $\theta$ and obtain the corresponding radii using the projection function $\mathcal{P}(\theta)$ (see \cref{fig:patch-partition}). The total number of patches is therefore $N_\varphi \times N_r$. In our experiments, we set $N_r=16$ and $N_\varphi = 64$ for an input image of size $64\times64$.

\subsection{Linear embedding}
\label{sec:linear-embedding}

The resulting image patches created by this approach have unequal amount of pixels. Therefore, we rely on a distortion aware sampling strategy to obtain the same number of points for each patch. To sample from the images, we define the number of sampling points along the radius and azimuth, and adapt the pattern according to each partition. In our experiments, we set 10 sampling points along radius and azimuth for each patch. Points are sampled in an equiangular fashion along the azimuth direction. For the radial dimension, we sample according to the same pattern as the polar partitioning (\cref{sec:polar-partition}); that is, we split in an equiangular fashion according to $\theta$ and obtain the corresponding radii using $\mathcal{P}(\theta)$. The input image is sampled using bilinear interpolation, and samples are arranged in a polar format \Ak{(for more information refer fig. 3 in supplementary)}. The resulting sample values are then fed into a linear embedding layer to produce token embeddings as input for the transformer block. 

% \begin{figure}[!h]
%   \centering
%   %\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%   \includegraphics[width=1.0\linewidth]{Figures/Darswin/Linear_embedding_1.pdf}
%   \caption{ \Ak{After the bi-linearly sampling layer, we use an MLP for linearly embedding patches. The illustration in this follows the \cref{fig:sampling} employs $N_r=2$ radius and $N_\varphi = 8$ azimuth partitions.}}
%   \label{fig:linear-embedding}
% \end{figure}

\subsection{Window-based self attention}
\label{sec:window-attn}
% \begin{figure}[t]
%   \centering
%   \footnotesize
%   \includegraphics[width=0.5\textwidth]{Figures/Darswin/before_shift.pdf} \\
%   (a) Window attention \\
%   \includegraphics[width=0.45\textwidth]{Figures/Darswin/after_shift.pdf} \\
%   (b) shifted window attention 
%   \caption[]{\todo{add caption for window shift}}
%   \label{fig:swinvdarswin}
% \end{figure}

The Swin transformer architecture~\cite{liu2021swin} uses window-based self-attention, where attention is computed on non-overlapping windows of $M\times M$ patches. Here, we maintain that strategy, but the polar nature of our patches allows us to define different numbers of patches along azimuth $M_\varphi$ and radius $M_r$. 
We define $M_\varphi = M^2$ patches along azimuth and $M_r = 1$ patch along radius. 
We experimentally found (see ablation in supplementary) that attention across $M^2$ patches along the azimuth yielded improved performance.

% gives us the following possibility to define different numbers of patches along different axis of the window ( $M_\varphi$ for the azimuth axis and $M_r$ for the radial axis), hence, the toal number of patches inside a window is $M_\varphi \times M_r = M^2$ as shown in \cref{tab:detailed architecture} 
%azimuth axis $M_\varphi$ and along radial axis $M_r$ and keeping the total number of patches in a window constant to $M^2$ as shown in \cref{tab:detailed architecture} 
% : we can either define $M$ patches along both azimuth and radius, $M_r = M_\varphi = M$ (DarSwin-RA), or we can define $M_\varphi = M^2$ patches along azimuth and $M_r = 1$ patch along radius (DarSwin-A). We found that computing attention across $M^2$ patches along the azimuth yielded greater performance, see \cref{sec:ablation}.



%Similar to Swin Transformer we can define $M$ patches along azimuth and radius, or we can define


%\todo{define $M_r$ and $M_\varphi$}, \Ak{we can take $M^2$ patches along the azimuth and  define windows entirely on azimuth (DarSwin-A), or we define $M$ patches on both radius and azimuth (DarSwin-RA), respectively, as shown in \cref{tab:detailed architecture}} \ola{The old sentence was clearer}. We found that computing attention across $M^2$ patches along the azimuth yielded greater performance, see \cref{sec:ablation}.

%Similarly, shifted window self-attention (used in \cite{liu2021swin} to introduce connections across windows at each stage of the network) is done by displacing the windows by $M$ patches along the azimuth.
% \todo{Explain how to shift the window using a figure}.

% In the swin transformer, the window self-attention block is followed by a \textbf{shifted window self-attention} block to introduce connection across windows, the second block receives windows shifted by $(\left\lfloor\frac{M}{2}\right\rfloor, \left\lfloor\frac{M}{2}\right\rfloor)$. In our method we use windows along azimuth, hence we use windows shifted along azimuth by $(1, M)$.

\begin{figure*}[!h]
\centering
\footnotesize
\setlength{\tabcolsep}{1pt}
\begin{tabular}{cccc}
\includegraphics[width=0.25\linewidth,trim=0 0 1cm 0,clip]{Figures/Classification/plot_gp0.pdf} & 

\includegraphics[width=0.25\linewidth,trim=0 0 1cm 0,clip]{Figures/Classification/plot_gp1.pdf} &

\includegraphics[width=0.25\linewidth,trim=0 0 1cm 0,clip]{Figures/Classification/plot_gp2.pdf} & 

\includegraphics[width=0.25\linewidth,trim=0 0 1cm 0,clip]{Figures/Classification/plot_gp3.pdf}
\\
(a) Very low & (b) Low & (c) Medium & (d) High
\end{tabular}
\caption[]{Top-1 classification accuracy (mean) as a function of test distortion for our method (\thename-A) and previous state of the art: DAT~\cite{xia2022vision}, Swin~\cite{liu2021swin}, and Swin (undis) (see text). All methods are trained on a restricted set of lens distortion curves (indicated by the pink shaded regions): (a) Very low, (b) low, (c) medium and (d) high distortion. We observe zero-shot adaptation to lens distortion of each approach by testing across all $\xi \in [0, 1]$.}
\label{fig:results-distortion}
\end{figure*}

\subsection{Angular relative positional encoding}
\label{sec:positional-encoding}

The Swin transformer relative positional encoding~\cite{liu2021swin} includes a position bias $B \in \mathbb{R}^{M^2 \times M^2}$, where $M^2$ is the number of patches in a window, added to each head when computing similarity: $\text{Att}(Q,K,V) = \text{Softmax}(QK^T / \sqrt{d} + B)V \,,$
%
% \begin{equation}
% \text{Att}(Q,K,V) = \text{Softmax}(QK^T / \sqrt{d} + B)V \,,
% \label{eq:attnswin}
% \end{equation}
%
where $Q,K,V$ $\in$ $\mathbb{R}^{M^2 \times d}$ are the queries, keys, and values matrices respectively; and $d$ is the query/key dimension. 

Since \thename follows a radial partitioning, we employ an angular relative positional encoding to capture the relative position between tokens with respect to incident $\theta$ and azimuth $\varphi$ angles.
We divide the position bias $B$ into two parts: $B_\theta$ and $B_\varphi$, the incident-angular and azimuthal relative position bias respectively. Given the $i$-th token angular coordinates $\theta_i = \frac{\theta_\mathrm{max} (i-0.5)}{N_r} \; \text{and} \;
\varphi_i = \frac{2\pi (i-0.5)}{N_\varphi} \,,$

%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{equation}
% \theta_i = \frac{\theta_\mathrm{max} (i-0.5)}{N_r} \; \text{and} \;
% \varphi_i = \frac{2\pi (i-0.5)}{N_\varphi} \,,
% \end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%
%
where $\theta_\mathrm{max}$ is the half field of view. The relative angular positions $(\Delta \theta, \Delta \varphi)$ between tokens $i,j$ are given by
%
\begin{align}
\Delta \theta &= \theta_i - \theta_j \,, \text{where} \, i,j \in [1, ..., N_\theta] \,, \text{and} \nonumber \\
% \theta_i - \theta_j &= \frac{\theta_{N_r}}{N_r} \,, \text{and}\nonumber \\
\Delta \varphi &= \varphi_i- \varphi_j \,, \text{where} \, i,j \in [1, ..., N_\varphi] \,.
\end{align}
%
%As in \cite{ning2020polar}, 
The tensors $B_\varphi$ and $B_\theta$ are defined as  $B_\theta = a_{\Delta \theta} \sin(\Delta \theta) + b_{\Delta \theta} \cos(\Delta \theta) \,, \text{ and }B_\varphi = a_{\Delta \varphi} \sin(\Delta \varphi) + b_{\Delta \varphi} \cos(\Delta \varphi) \,.$
% based on the relative values $\Delta \theta$ and $\Delta \varphi$ of each .
%
% \begin{align}
%   B_\theta &= a_{\Delta \theta} \sin(\Delta \theta) + b_{\Delta \theta} \cos(\Delta \theta) \,, \\
%   %+ \frac{1}{P}\sum\limits_{p=1}^P(a_{r, p}\cos \frac{2\pi p \Delta r}{r_\mathrm{max}} + b_{r, p}\sin \frac{2\pi p \Delta r}{r_\mathrm{max}}) \,, \nonumber \\
% B_\varphi &= a_{\Delta \varphi} \sin(\Delta \varphi) + b_{\Delta \varphi} \cos(\Delta \varphi) \,.
%   %f_\varphi(\Delta \varphi) &= a_{\varphi, 0} + \frac{1}{P}\sum\limits_{p=1}^P(a_{\varphi, p}\cos p \Delta \varphi + b_{\varphi, p}\sin p \Delta \varphi) \,. 
%   \label{eq:positional-encoding}
% \end{align}
%

Here, $a_*$ and $b_*$ are trainable coefficients. Since the relative positions in a window along angular and azimuth axes ranges from $[-M_\theta + 1, M_\theta - 1]$ and $[-M_\varphi + 1, M_\varphi - 1]$ respectively, where $M_\theta$ and $M_\varphi$ are number of patches in a window (see \cref{sec:window-attn}, here $M_\theta=M_r$). We parameterize two bias matrices $\hat{B}_\varphi \in \mathbb{R}^{(2M_\varphi - 1) \times 2}$ and $\hat{B}_r \in \mathrm{R}^{(2M_\theta - 1) \times 2}$. Hence $a_*$ and $b_*$ are taken from $\hat{B}_\theta$ and $\hat{B}_\varphi$.

% Here, $r_\mathrm{max}$ is the half image size, $a_*$ and $b_*$ are trainable coefficient vectors, and $P$ controls the number of higher frequency components used---there are therefore $4P + 2$ such coefficients in total. In our experiments, we set $P=4$.

Finally, the two tensors $B_\theta,B_\varphi \in \mathbb{R}^{M_r^2 \times M_\varphi^2}$ are built on all pairs of tokens. The final attention equation is thus $\text{Att}(Q,K,V) = \text{Softmax}(QK^T / \sqrt{d} + B_\theta + B_\varphi)V \,.$
    \label{eq:attention}
%
% \begin{equation}
%     \text{Att}(Q,K,V) = \text{Softmax}(QK^T / \sqrt{d} + B_\theta + B_\varphi)V \,.
%     \label{eq:attention}
% \end{equation}

% \begin{figure}[!h]
%   \centering
%   %\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%   \includegraphics[width=1.00\linewidth]{Figures/Darswin/Positional_encoding.pdf}
%   \caption{Example of polar position encoding we use to define positions of each patch in the radius-azimuth format. We define relative azimuth and radial position of each patch with respect to every other patch to get position bias $\mathit{B}_\mathit{r}$ and $\mathit{B}_\varphi$ respectively. }
%   \label{fig:RPE}
% \end{figure}

\subsection{Polar patch merging}
\label{sec:patch-merging}

Similar to window-based self attention (\cref{sec:window-attn}), the polar nature of our architecture enables many possibilities when merging patches. For example, we found that merging $1 \times 4$ patches along azimuth (\thename-A)outperform the others in our experiments \Ak{(see ablations in supplementary).}

% \begin{table}
% \centering
% \caption{Model architecture specification and variants. DarSwin-RA: merging  $2\times2$ neighborhood patches along the radius and azimuth, DarSwin-A: merging $1\times4$ neighborhood patches along the azimuth . $N_r$ and $N_\varphi$ denote the number of patches along azimuth and radius. $n_a \text{ and } n_r$: denote the number of sampling points along radius and azimuth. $P$ frequency parameter for polar positional encoding. $B_i$: number of blocks at stage$_i$, window: window size, the region of local attention module and heads: number of heads in shifted window multi-head self-attention (SW-MHSA)}
% \begin{tabular}{ccc} 
% \toprule
% \begin{tabular}[c]{@{}c@{}}$N_r$ = 16, $N_\varphi$ = 64\\$n_r$ = $n_a$ = 10\\$P$ = 4\end{tabular} & \begin{tabular}[c]{@{}c@{}}Darswin-RA\\window= (4, 4)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Darswin-A\\window= (1,16)\end{tabular}  \\ 
% \hline
% \begin{tabular}[c]{@{}c@{}}$B_1$ = 2, C = 96\\heads = 3\end{tabular}                     & \begin{tabular}[c]{@{}c@{}}Stage 1\\(16, 64)\end{tabular}               & \begin{tabular}[c]{@{}c@{}}Stage 1\\(16, 64)\end{tabular}                \\ 
% \hline
% \begin{tabular}[c]{@{}c@{}}$B_2$ = 2, C = 192\\heads = 6\end{tabular}                     & \begin{tabular}[c]{@{}c@{}}Stage 2\\(8, 32)\end{tabular}                & \begin{tabular}[c]{@{}c@{}}Stage 2\\(16, 16)\end{tabular}                \\ 
% \hline
% \begin{tabular}[c]{@{}c@{}}$B_3$ = 18, C = 384\\heads = 12\end{tabular}                     & \begin{tabular}[c]{@{}c@{}}Stage 3\\(4, 16)\end{tabular}                & \begin{tabular}[c]{@{}c@{}}Stage 3\\(16, 4)\end{tabular}                 \\ 
% \hline
% \begin{tabular}[c]{@{}c@{}}$B_4$ = 2, C = 768\\heads = 24\end{tabular}                     & \begin{tabular}[c]{@{}c@{}}Stage 4\\(2,8)\end{tabular}                  & \begin{tabular}[c]{@{}c@{}}Stage 4\\(16, 1)\end{tabular}                 \\
% \bottomrule
% \end{tabular}
% \label{tab:detailed architecture}
% \end{table}


% \begin{table}[]
% \footnotesize
% \centering
% \caption{\Ak{Model architecture specification and variants. In both variants, we adapt the small architecture of Swin Transformer \cite{liu2021swin}, which has four stages of patch merging. \textbf{Input Resolution} : Resolution of feature map at every stage. \textbf{Window Size} : Window size ($M_r, M_\varphi$), $M_r$ : Number of patches along radial axis in a window, $M_\varphi$ : Number of patches along azimuth axis in a window. \textbf{DarSwin-RA}: Architecture variant with four patches along both azimuth and radial axis and merging $2 \times 2$ neighborhood patches along the radius and azimuth. \textbf{DarSwin-A}: architecture variant with 16 patches along the azimuth axis and one patch along the radial axis in a window and merging $1 \times 4$ neighborhood patches along the radius and azimuth.}}
% \begin{tabular}{cccc}
% \hline
% \multicolumn{2}{c}{DarSwin-RA}                                                                                                                                      & \multicolumn{2}{c}{DarSwin-A}                                                                                                                                       \\ \hline
% \begin{tabular}[c]{@{}c@{}}Input Resolution\end{tabular} & \begin{tabular}[c]{@{}c@{}}Window Size\\ $(M_r, M_\varphi)$\end{tabular} & \begin{tabular}[c]{@{}c@{}}Input Resolution\end{tabular} & \begin{tabular}[c]{@{}c@{}}Window Size\\ $(M_r, M_\varphi)$\end{tabular} \\ \hline
% \begin{tabular}[c]{@{}c@{}}Stage-1\\ (16, 64)\end{tabular}                & (4, 4)                                                                                  & \begin{tabular}[c]{@{}c@{}}Stage-1\\ (16, 64)\end{tabular}                & (1, 16)                                                                                 \\ \hline
% \begin{tabular}[c]{@{}c@{}}Stage-2\\ (8, 32)\end{tabular}                 & (4, 4)                                                                                  & \begin{tabular}[c]{@{}c@{}}Stage-2\\ (16, 16)\end{tabular}                & (1, 16)                                                                                 \\ \hline
% \begin{tabular}[c]{@{}c@{}}Stage-3\\ (4, 16)\end{tabular}                 & (4, 4)                                                                                  & \begin{tabular}[c]{@{}c@{}}Stage-3\\ (16, 4)\end{tabular}                 & (4, 4)                                                                                  \\ \hline
% \begin{tabular}[c]{@{}c@{}}Stage-4\\ (2, 8)\end{tabular}                  & (2, 8)                                                                                  & \begin{tabular}[c]{@{}c@{}}Stage-4\\ (16, 1)\end{tabular}                 & (16, 1)                                                                                 \\ \hline
% \end{tabular}
% \label{tab:detailed architecture}
% \end{table}





==> Sections_workshop/related_works_workshop.tex <==
%!TEX root = ../main.tex
\section{Related work}

% Unlike convolutional-based networks ~\cite{dai2017deformable, zhu2019deformable}, our work falls within proposing a novel transformer-based~\cite{vaswani2017attention, dosovitskiy2020image, liu2021swin} representation learning,  approaches for wide-angle image classification and segmentation. The followings are highly related works from convolution- and transformer-based approaches, besides the wide-angle works \cite{jang2022dada,yun2022panoramic,zhang2022bending}. 

% \paragraph{Panoramic distortion} Panoramic images span the full \ang{360} field of view and are most commonly projected onto a plane using an equirectangular projection creates severe distortions especially near the poles. Many works have explicitly designed approaches to deal with equirectangular distortion, including depth estimation~\cite{zioulis2018omnidepth}, saliency detection~\cite{yun2022panoramic}, segmentation~\cite{zhang2022bending}, layout estimation~\cite{fernandez2018layouts}, and object detection~\cite{su2019kernel} to name a few. However, as with \cite{cohen2018spherical}, these are specifically designed for spherical distortion and do not generalize to wide-angle lenses. 


%\paragraph{Wide angle} 
\paragraph{Image undistortion}
Applying tasks like classification and object recognition on wide-angle images is relatively recent~\cite{Rashed_2021_WACV,inproceedings,plaut2021fisheye, Ye2020UniversalSS, yogamani2019woodscapes} due to the presence of distortions in the image. In computer vision, the application of wide-angle images ranges from visual perception~\cite{kumar2021omnidet} to autonomous vehicle cameras~\cite{yogamani2019woodscapes, kumar2022surround, liao2022kitti}. In this respect, the initial studies mainly focused on correcting the distortion of the image \cite{xue2019learning, article1, yin2018fisheyerectnet, zhang2015line, 9980359}. Recently, many convolutional-based and attention-based models have been proposed that try to directly reason on wide-angle images without relying on distortion correction models. 

% \subsection{Deformable CNN or CNN methods and explain the use of transformer}
% \ola{I would split this paragraph and not mix convolution with vision transformer}
% \paragraph{Deformable convolutions and vision transformer} 
% \paragraph{Convolution-based approaches} 
% CNNs~\cite{krizhevsky2012classif, VGG, googlenet} are particularly well-suited for perspective images due to their implicit bias and translational equivariance \cite{GDL}. Methods like \cite{8500456, inproceedings, Rashed_2021_WACV} tries to adapt CNNs on fisheye images for tasks such as object detection. However, the distortion caused by wide angle images breaks this symmetry, which reduces the generalization performance of CNNs. Deformable convolutions~\cite{dai2017deformable} (later extended in \cite{zhu2019deformable}) learn a deformation to be applied to convolution kernels which can provide greater flexibility at the cost of significant additional computation. Closer to our work, \cite{ahmad2022fisheyehdk, playout2021adaptable,deng2019restricted} use such deformable CNNs to understand the distortion in a fisheye image. In contrast, our \thename leverages attention-based mechanisms rather than convolution. Recently, Jang et al.~\cite{jang2022dada} proposed a framework for distortion-aware domain adaptation, where a generator network is trained to transform an image to a different lens profile. In contrast, our method can adapt to a different lens without additional training. 

% hence many methods like Deformable CNN based architecture \cite{dai2017deformable, zhu2019deformable} 
% try to enhance the geometric representational learninig ability of the CNN by 

% using deforming kernels in the building modules of CNN. Specifically, Dia~\etal~\cite{dai2017deformable} proposed deformable convolutions by augmenting spacial sampling through the additional offset learning. Thereafter, Zhu~\etal~\cite{zhu2019deformable} expanded the deformable convolutions with more convolution layers to increase the ability of sampling over a large range of features. 
% Methods like 
% \cite{ahmad2022fisheyehdk, playout2021adaptable} 
% uses deformable CNNs to understand the distortion in a fisheye image. However, unlike grid-based deformable convolutions~\cite{dai2017deformable, zhu2019deformable}, our DarSwin is radial-based and is built on recent advances in attention-based~\cite{vaswani2017attention} geometric transformation learning. 

\paragraph{Self-attention-based approaches} Vision transformers (ViT)~\cite{dosovitskiy2020vit} use self-attention mechanisms~\cite{vaswani2017attention} computed on image patches rather than performing convolutions. Unlike CNNs, a ViT does not have a fixed geometric structure in its architecture: any extra structure is given via positional encoding. More recently, the Swin transformer architecture~\cite{liu2021swin} proposes a multi-scale strategy of window-based attention. Later, deformable attention transformer (DAT)~\cite{xia2022vision}, adapts the concept of deformable CNNs~\cite{dai2017deformable,zhu2019deformable} to increase adaptability. Unlike existing transformer architectures, \thename explicitly embeds the distortion into its structure using polar sampling, patch partition, window-based self-attention, and angular positional encoding. 


% Saliency detection in \ang{360} videos using panoramic transformer~\cite{yun2022panoramic} is another vision task to employ wide-angle images. In particular, they proposed panoramic vision transformer (PAVER)~\cite{yun2022panoramic}, a hybrid deformable-based transformer-convolution method to estimate the geometric approximation However, unlike our DarSwin, PAVER is restricted \ang{360} inputs (a sphere) and not fisheye.  %They use spherical projection (Equirectangular projection which is a one-to-one mapping from a sphere to a rectangle then apply a bunch of modules - transformer and deformable conv.)  
% \ola{this method is restricted to 360 degree inputs (a sphere) and not fisheye. Fisheye is not a perfect sphere. They use spherical projection (Equirectangular projection which is a one-to-one mapping from sphere to rectangle then apply a bunch of modules - transformer and deformable conv.)}. 

% From the ``distortion-aware'' perspective, our method is also related to panoramic segmentation~\cite{zhang2022bending}, where they adapt transformers to learn both object deformations and panoramic image distortions with dual deformable patch embedding and deformable MLP modules. However, in contrast to~\cite{zhang2022bending}, our DarSwin extends beyond the panoramic input images and generalizes to distortion-aware via radial patch embedding function.

% Adapting to panoramic segmentation~\cite{zhang2022bending}---very important to address carefully since they also claim ``distortion-aware''.\ola{I dont think we need to focus too much on the task here but the techniques and their limitations. The work in [36] is also limited to panoramic images. Distortions are created because of the equirectangular projection and not because of the lens itself.}






% As an alternative approach to CNNs, Vaswani~\etal~\cite{vaswani2017attention} proposed transformers to apply self-attention mechanism for language modeling. Afterward, Dosovitskiy~\etal~\cite{dosovitskiy2020image} proposed vision transformers (ViT) for computer vision tasks the motivation behind introducing a transformer in a CNN-dominated field was the expressivity of the network. 
% This increased degree of freedom enables the transformer to find a very original and unexpected way to look at data, given a large amount of data. 
% Furthermore, Liu~\etal\cite{liu2021swin} proposed Swin transformer, which contains the shifted windowing to enhance ViT for capturing the cross-window connection. In particular, they aim to capture the variant scale modeling of input images using a hierarchical architecture of the Swin. 
% Deformable attention transformer (DAT) \cite{xia2022vision}, adapts the concept of deformable CNNs in vision transformer to increase the where, a deformable self-attention mechanism is proposed to specify the appropriate position of key and value at the time of attention. Our DarSwin which is highly related to Swin \cite{liu2021swin} aims at enhancing the geometric transformation capability of the vision transformers to the wide-angle input images by adapting Swin blocks proposed by \cite{liu2021swin}. 





 
% \subsection{Swin, DAT}
% \paragraph{Swin and deformable transformer}
% Swin
%  However, our DarSwin proposes a novel radial patch
% partitioning for adapting to the lens distortion profile.  \todo{discuss DAT}  

%\todo{discuss the difference between Swin and DarSwin}            
 
% DAT






% \subsection{Wide angle}





==> notes.tex <==
\section{Notes}
\listoftodos

Papers are limited to eight pages, including figures and tables, in the ICCV style. Additional pages containing only cited references are allowed. Appendices may not be a part of the additional pages. Appendices are counted towards the eight-page limit or should be moved to the supplementary document. Please refer to the following files for detailed formatting instructions:

\begin{enumerate}
    \item Appendix
    \item Supplemental Material
    \begin{enumerate}
        \item loss curves
    \end{enumerate}
\end{enumerate}
